Measurement of isotopic separation of argon with the prototype of the cryogenic distillation plant Aria for dark matter searches

The Aria cryogenic distillation plant, located in Sardinia, Italy, is a key component of the DarkSide-20k experimental program for WIMP dark matter searches at the INFN Laboratori Nazionali del Gran Sasso, Italy. Aria is designed to purify the argon, extracted from underground wells in Colorado, USA, and used as the DarkSide-20k target material, to detector-grade quality. In this paper, we report the first measurement of argon isotopic separation by distillation with the 26 m tall Aria prototype. We discuss the measurement of the operating parameters of the column and the observation of the simultaneous separation of the three stable argon isotopes: Ar$^{36}$, Ar$^{38}$, and Ar$^{40}$. We also provide a detailed comparison of the experimental results with commercial process simulation software. This measurement of isotopic separation of argon is a significant achievement for the project, building on the success of the initial demonstration of isotopic separation of nitrogen using the same equipment in 2019.

==> basic/author_list_end.tex <==

% \renewcommand{\thanksref}[1]{$^{\ref{#1}}$}
%\newcommand{\notds}{\nolinebreak\footnotemark\nolinebreak}
%\renewcommand{\thefootnote}{$*$}

%{
%\onecolumn
% \textbf{The Aria and DarkSide-20k Collaborations}%
%\textbf{The DarkSide-20k Collaboration}
%\footnotetext{Not a member of the DarkSide-20k Collaboration}

% \newline
%P.~Agnes\thanksref{Houston}\nolinebreak, 
%S.~Albergo\thanksref{CTINFN}{CTUNI}\nolinebreak, 
%I.~F.~M.~Albuquerque\thanksref{USP}\nolinebreak,
%T.~Alexander\thanksref{PNNLaddress}\nolinebreak,
%A.~Alici\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
%A.~K.~Alton\thanksref{Augustana}\nolinebreak,
%P.~Amaudruz\thanksref{TRIUMFaddress}\nolinebreak,
M.~Arba\thanksref{CAINFN}\nolinebreak,
%P.~Arpaia\thanksref{NAUniPHY}\nolinebreak,
%S.~Arcelli\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
%M.~Ave\thanksref{USP}\nolinebreak,
%% I.~Ch.~Avetissov\thanksref{MendeleevUniverisity}\nolinebreak,
%R.~I.~Avetisov\thanksref{MendeleevUniverisity}\nolinebreak,
%O.~Azzolini\thanksref{LNLINFN}\nolinebreak,
%H.~O.~Back\thanksref{PNNLaddress}\nolinebreak,
%Z.~Balmforth\thanksref{RHUL}\nolinebreak,
%V.~Barbarian\thanksref{MSU}\nolinebreak,
%A.~Barrado~Olmedo\thanksref{CIEMAT}\nolinebreak,
%~P.~Barrillon\thanksref{CPPM}\nolinebreak,
%A.~Basco\thanksref{NAINFN}\nolinebreak,
%G.~Batignani\thanksref{PIINFN}{PIUniPHY}\nolinebreak,
%A.~Bondar\thanksref{BINP}{NSU}\nolinebreak,
W.~M.~Bonivento\thanksref{CAINFN}\nolinebreak,
%E.~Borisova\thanksref{BINP}{NSU}\nolinebreak,
%B.~Bottino\thanksref{GEUni}{GEINFN}\nolinebreak,
%M.~G.~Boulay\thanksref{Carleton}\nolinebreak,
%G.~Buccino\thanksref{CERNaddress}\nolinebreak,
%S.~Bussino\thanksref{RMTreINFN}{RMTreUni}\nolinebreak,
%J.~Busto\thanksref{CPPM}\nolinebreak,
%A.~Buzulutskov\thanksref{BINP}{NSU}\nolinebreak,
M.~Cadeddu\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
%M.~Cadoni\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
%A.~Caminata\thanksref{GEINFN}\nolinebreak,
%E.V.~Canesi\thanksref{Polaris}\notds\nolinebreak,
%N.~Canci\thanksref{AQLNGS}\nolinebreak,
%G.~Cappello\thanksref{CTINFN}{CTUNI}\nolinebreak,
M.~Caravati\thanksref{CAINFN}\nolinebreak,
%M.~C\'ardenas-Montes\thanksref{CIEMAT}\nolinebreak,
N.~Cargioli\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
%M.~Carlini\thanksref{AQGSSI}\nolinebreak,
%F.~Carnesecchi\thanksref{BOINFN}{BOUniPHY}\nolinebreak,
P.~Castello\thanksref{CAUniEEE}{CAINFN}\nolinebreak,
%A.~Castellani\thanksref{MIPoliICA}\nolinebreak,
%S.~Catalanotti\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
%V.~Cataudella\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
P.~Cavalcante\thanksref{AQLNGS}\nolinebreak,
%5S.~Cavuoti\thanksref{NAUniPHY}{NAINFN}{OACINAF}\nolinebreak,
%S.~Cebrian\thanksref{Zaragoza}\nolinebreak,
%J.~M.~Cela~Ruiz\thanksref{CIEMAT}\nolinebreak,
%B.~Celano\thanksref{NAINFN}\nolinebreak,
%S.~Chashin\thanksref{MSU}\nolinebreak,
%A.~Chepurnov\thanksref{MSU}\nolinebreak,
%C.~Cical\`o\thanksref{CAINFN}\nolinebreak,
%L.~Cifarelli\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
%D.~Cintas\thanksref{Zaragoza}\nolinebreak,
%F.~Coccetti\thanksref{CentroFermi}\nolinebreak,
V.~Cocco\thanksref{CAINFN}\nolinebreak,
%M.~Colocci\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
%E.~Conde~Vilda\thanksref{CIEMAT}\nolinebreak,
%L.~Consiglio\thanksref{AQLNGS}\nolinebreak,
%S.~Copello\thanksref{GEINFN}{GEUni}\nolinebreak,
%J.~Corning\thanksref{Queens}\nolinebreak,
%G.~Covone\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
%P.~Czudak\thanksref{Krakow}\nolinebreak,
%M.~D'Aniello\thanksref{NAUniStruct}\nolinebreak,
%S.~D'Auria\thanksref{MIINFN}\nolinebreak,
%M.~D.~Da~Rocha~Rolo\thanksref{TOINFN}\nolinebreak,
%O.~Dadoun\thanksref{LPNHE}\nolinebreak,
%M.~Daniel\thanksref{CIEMAT}\nolinebreak,
%S.~Davini\thanksref{GEINFN}\nolinebreak,
%A.~De~Candia\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
%S.~De~Cecco\thanksref{RMUnoINFN}{RMUnoUni}\nolinebreak,
%A.~De~Falco\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
%G.~De~Filippis\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
%D.~De~Gruttola\thanksref{SAUni}{SAINFN}\nolinebreak,
%G.~De~Guido\thanksref{MIPoliCHE}\nolinebreak,
%G.~De~Rosa\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
%M.~Della~Valle\thanksref{NAINFN}{OACINAF}\nolinebreak,
%G.~Dellacasa\thanksref{TOINFN}\nolinebreak,
%S.~De Pasquale\thanksref{SAUni}{SAINFN}\nolinebreak,
%A.~V.~Derbin\thanksref{Petersburg}\nolinebreak,
A.~Devoto\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
%L.~Di~Noto\thanksref{GEINFN}\nolinebreak,
%F.~Di Eusanio\thanksref{Princeton}\nolinebreak,
%C.~Dionisi\thanksref{RMUnoINFN}{RMUnoUni}\nolinebreak,
%P.~Di Stefano\thanksref{Queens}\nolinebreak,
%G.~Dolganov\thanksref{Kurchatov}\nolinebreak,
%D.~Dongiovanni\thanksref{ENEA}\nolinebreak,
F.~Dordei\thanksref{CAINFN}\nolinebreak,
%M.~Downing\thanksref{UMass}\nolinebreak,
%T.~Erjavec\thanksref{UCDavis}\nolinebreak,
%S.~Falciano\thanksref{AQGSSI}{RMUnoINFN}\nolinebreak,
%S.~Farenzena\thanksref{CS}\notds\nolinebreak,
%M.~Fernandez~Diaz\thanksref{CIEMAT}\nolinebreak,
%C.~Filip\thanksref{INCDTIM}\nolinebreak,
%G.~Fiorillo\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
%A.~Franceschi\thanksref{LNFINFN}\nolinebreak,
%D.~Franco\thanksref{APC}\nolinebreak,
%E.~Frolov\thanksref{BINP}{NSU}\nolinebreak,
N.~Funicello\thanksref{SAUni}{SAINFN}\nolinebreak,
F.~Gabriele\thanksref{AQLNGS}\nolinebreak,
C.~Galbiati\thanksref{Princeton}{AQLNGS}{AQGSSI}\nolinebreak,
%M.~Garbini\thanksref{CentroFermi}{BOINFN}\nolinebreak,
%P.~Garcia~Abia\thanksref{CIEMAT}\nolinebreak,
%A.~Gendotti\thanksref{ETHZ}\nolinebreak,
%C.~Ghiano\thanksref{AQLNGS}\nolinebreak,
%R.~A.~Giampaolo\thanksref{TOINFN}{TOPoli}\nolinebreak,
%C.~Giganti\thanksref{LPNHE}\nolinebreak,
%M.~A.~Giorgi\thanksref{PIUniPHY}{PIINFN}\nolinebreak,
%G.~K.~Giovanetti\thanksref{WilliamsCollege}\nolinebreak,
%M.L.~Gligan\thanksref{INCDTIM}\nolinebreak,
%V.~Goicoechea~Casanueva\thanksref{Hawaii}\nolinebreak,
%A.~Gola\thanksref{TNFBK}{TNTIFPA}\nolinebreak,
%A.M.~Goretti\thanksref{AQLNGS}\nolinebreak,
%R.~Graciani~Diaz\thanksref{UB}\nolinebreak,
%G.~Y.~Grigoriev\thanksref{Kurchatov}\nolinebreak,
%A.~Grobov\thanksref{Kurchatov}{MEPhI}\nolinebreak,
%M.~Gromov\thanksref{MSU}{JINR}\nolinebreak,
%M.~Guan\thanksref{IHEPaddress}\nolinebreak,
%M.~Guerzoni\thanksref{BOINFN}\nolinebreak,
M.~Guetti\thanksref{AQLNGS}\nolinebreak,
%M.~Gulino\thanksref{ENUniCEE}{CTLNS}\nolinebreak,
%C.~Guo\thanksref{IHEPaddress}\nolinebreak,
%B.~R.~Hackett\thanksref{PNNLaddress}\nolinebreak,
%A.~Hallin\thanksref{Alberta}\nolinebreak,
%M.~Haranczyk\thanksref{Krakow}\nolinebreak,
%S.~Hill\thanksref{RHUL}\nolinebreak,
%S.~Horikawa\thanksref{AQGSSI}{AQLNGS}\nolinebreak,
%F.~Hubaut\thanksref{CPPM}\nolinebreak,
%.~Hugues\thanksref{AstroCeNT}\nolinebreak,
%E.~V.~Hungerford\thanksref{Houston}\nolinebreak,
%An.~Ianni\thanksref{Princeton}{AQLNGS}\nolinebreak,
%V.~Ippolito\thanksref{RMUnoINFN}\nolinebreak,
%C.~C.~James\thanksref{FNALaddress}\nolinebreak,
%C.~Jillings\thanksref{SNOLABaddress}{Laurentian}\nolinebreak,
%P.~Kachru\thanksref{AQGSSI}{AQLNGS}\nolinebreak%,
%A.~A.~Kemp\thanksref{Queens}\nolinebreak,
C.~L.~Kendziora\thanksref{FNALaddress}\nolinebreak,
%G.~Keppel\thanksref{LNLINFN}\nolinebreak,
%A.~V.~Khomyakov\thanksref{MendeleevUniverisity}\nolinebreak,
% S.~Kim\thanksref{Temple}\nolinebreak,
M.~Kimura\thanksref{AstroCeNT}\nolinebreak,
%A.~Kish\thanksref{Hawaii}\nolinebreak,
%I.~Kochanek\thanksref{AQLNGS}\nolinebreak,
%.~Kondo\thanksref{AQLNGS}\nolinebreak,
%G.~Korga\thanksref{RHUL}\nolinebreak,
%A.~Kubankin\thanksref{Belgorod}\nolinebreak,
%R.~Kugathasan\thanksref{TOINFN}{TOPoli}\nolinebreak,
%M.~Kuss\thanksref{PIINFN}\nolinebreak,
%M.~Kuźniak\thanksref{AstroCeNT}\nolinebreak,
%M.~La~Commara\thanksref{NAUniPHARM}{NAINFN}\nolinebreak,
L.~La Delfa\thanksref{CAINFN}\nolinebreak,
%D.~La Grasta\thanksref{Polaris}\notds\nolinebreak,
M.~Lai\thanksref{CAUniPHY}{CAINFN}{APC}\nolinebreak,
%N.~Lami\thanksref{CS}\notds\nolinebreak,
%S.~Langrock\thanksref{Laurentian}\nolinebreak,
%M.~Leyton\thanksref{NAINFN}\nolinebreak,
%X.~Li\thanksref{Princeton}\nolinebreak,
%L.~Lidey\thanksref{PNNLaddress}\nolinebreak,
%F.~Lippi\thanksref{CS}\notds\nolinebreak,
%M.~Lissia\thanksref{CAINFN}\nolinebreak,
%G.~Longo\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
%N.~Maccioni\thanksref{CS}\notds\nolinebreak,
%I.~N.~Machulin\thanksref{Kurchatov}{MEPhI}\nolinebreak,
%L.~Mapelli\thanksref{Princeton}\nolinebreak,
%A.~Marasciulli\thanksref{PIUniPHY}\nolinebreak,
%A.~Margotti\thanksref{BOINFN}\nolinebreak,
%S.~M.~Mari\thanksref{RMTreINFN}{RMTreUni}\nolinebreak,
%J.~Maricic\thanksref{Hawaii}\nolinebreak,
%M.~Marinelli\thanksref{GEINFN}\nolinebreak,
%M.~Mart\'inez\thanksref{Zaragoza}{ZaragozaARAID}\nolinebreak,
%A.~D.~Martinez~Rojas\thanksref{TOINFN}{TOPoli}\nolinebreak,
%A.~Martini\thanksref{CS}{MISE}\notds\nolinebreak,
% C.~J.~Martoff\thanksref{Temple}\nolinebreak,
%M.~Mascia\thanksref{CAUniCHE}\nolinebreak,
%M.~Masetto\thanksref{Polaris}\notds\nolinebreak,
A.~Masoni\thanksref{CAINFN}\nolinebreak,
%A.~Mazzi\thanksref{TNFBK}{TNTIFPA}\nolinebreak,
%A.~B.~McDonald\thanksref{Queens}\nolinebreak,
%J.~Mclaughlin\thanksref{TRIUMFaddress}{RHUL}\nolinebreak,
%A.~Messina\thanksref{RMUnoINFN}{RMUnoUni}\nolinebreak,
%P.~D.~Meyers\thanksref{Princeton}\nolinebreak,
%T.~Miletic\thanksref{Hawaii}\nolinebreak,
%R.~Milincic\thanksref{Hawaii}\nolinebreak,
%R.~Miola\thanksref{Polaris}\notds\nolinebreak,
%.~Moggi\thanksref{PIINFN}\nolinebreak,
%A.~Moharana\thanksref{AQGSSI}{AQLNGS}\nolinebreak,
%S.~Moioli\thanksref{MIPoliCHE}\nolinebreak,
%J.~Monroe\thanksref{RHUL}\nolinebreak,
%S.~Morisi\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
%M.~Morrocchi\thanksref{PIINFN}{PIUniPHY}\nolinebreak,
%E.~N.~Mozhevitina\thanksref{MendeleevUniverisity}\nolinebreak,
%T.~Mr\'oz\thanksref{Krakow}\nolinebreak,
%V.~N.~Muratova\thanksref{Petersburg}\nolinebreak,
%A.~Murenu\thanksref{CAINFN}\nolinebreak,
%C.~Muscas\thanksref{CAUniEEE}{CAINFN}\nolinebreak,
%L.~Musenich\thanksref{GEINFN}{GEUni}\nolinebreak,
%P.~Musico\thanksref{GEINFN}\nolinebreak,
%R.~Nania\thanksref{BOINFN}\nolinebreak,
%T.~Napolitano\thanksref{LNFINFN}\nolinebreak,
%A.~Navrer~Agasson\thanksref{LPNHE}\nolinebreak,
%M.~Nessi\thanksref{CERNaddress}\nolinebreak,
%I.~Nikulin\thanksref{Belgorod}\nolinebreak,
S.~Nisi\thanksref{AQLNGS}\nolinebreak,
%J.~Nowak\thanksref{Lancaster}\nolinebreak,
%A.~Oleinik\thanksref{Belgorod}\nolinebreak,
%V.~Oleynikov\thanksref{BINP}{NSU}\nolinebreak,
%L.~Pagani\thanksref{UCDavis}\nolinebreak,
%M.~Pallavicini\thanksref{GEUni}{GEINFN}\nolinebreak,
%S.~Palmas\thanksref{CAUniCHE}\nolinebreak,
%L.~Pandola\thanksref{CTLNS}\nolinebreak,
%E.~Pantic\thanksref{UCDavis}\nolinebreak,
%E.~Paoloni\thanksref{PIINFN}{PIUniPHY}\nolinebreak,
%G.~Paternoster\thanksref{TNFBK}{TNTIFPA}\nolinebreak,
%P.~A.~Pegoraro\thanksref{CAUniEEE}{CAINFN}\nolinebreak,
%L.~A.~Pellegrini\thanksref{MIPoliCHE}\nolinebreak,
%C.~Pellegrino\thanksref{BOINFN}\nolinebreak,
%K.~Pelczar\thanksref{Krakow}\nolinebreak,
%F.~Perotti\thanksref{MIPoliICA}{MIINFN}\nolinebreak,
%V.~Pesudo\thanksref{CIEMAT}\nolinebreak,
%E.~Picciau\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
%F.~Pietropaolo\thanksref{CERNaddress}\nolinebreak,
%T.~Pinna\thanksref{ENEA}\nolinebreak,
%.~Pocar\thanksref{UMass}\nolinebreak,
%.~Podda\thanksref{CS}\notds\nolinebreak,
%D.~M.~Poehlmann\thanksref{UCDavis}\nolinebreak,
%S.~Pordes\thanksref{FNALaddress}\nolinebreak,
%S.~S.~Poudel\thanksref{Houston}\nolinebreak,
%P.~Pralavorio\thanksref{CPPM}\nolinebreak,
%D.~Price\thanksref{Manchester}\nolinebreak,
%F.~Raffaelli\thanksref{PIINFN}\nolinebreak,
%F.~Ragusa\thanksref{MIUni}{MIINFN}\nolinebreak,
%A.~Ramirez\thanksref{Houston}\nolinebreak,
%M.~Razeti\thanksref{CAINFN}\nolinebreak,
%A.~Razeto\thanksref{AQLNGS}\nolinebreak,
%A.~L.~Renshaw\thanksref{Houston}\nolinebreak,
%S.~Rescia\thanksref{BNLaddress}\nolinebreak,
%M.~Rescigno\thanksref{RMUnoINFN}\nolinebreak,
%F.~Resnati\thanksref{CERNaddress}\nolinebreak,
%F.~Retiere\thanksref{TRIUMFaddress}\nolinebreak%,
%L.~P.~Rignanese\thanksref{BOINFN}{BOUniPHY}\nolinebreak,
%C.~Ripoli\thanksref{SAINFN}{SAUni}\nolinebreak,
%A.~Rivetti\thanksref{TOINFN}\nolinebreak,
%J.~Rode\thanksref{LPNHE}{APC}\nolinebreak,
%L.~Romero\thanksref{CIEMAT}\nolinebreak,
%M.~Rossi\thanksref{GEINFN}{GEUni}\nolinebreak,
%A.~Rubbia\thanksref{ETHZ}\nolinebreak,
%M.~Rucaj\thanksref{Polaris}\notds\nolinebreak,
%G.M.~Sabiu\thanksref{CS}\notds\nolinebreak,
%P.~Salatino\thanksref{NAUniCHE}{NAINFN}\nolinebreak,
%O.~Samoylov\thanksref{JINR}\nolinebreak,
%E.~S\'anchez~Garc\'ia\thanksref{CIEMAT}\nolinebreak,
%E.~Sandford\thanksref{Manchester}\nolinebreak,
%S.~Sanfilippo\thanksref{RMTreUni}{RMTreINFN}\nolinebreak,
%V.A.~Sangiorgio\thanksref{MIPoliCHE}\nolinebreak,
%V.~Santacroce\thanksref{CS}\notds\nolinebreak,
%D.~Santone\thanksref{RHUL}\nolinebreak,
%R.~Santorelli\thanksref{CIEMAT}\nolinebreak,
%A.~Santucci\thanksref{ENEA}\nolinebreak,
%C.~Savarese\thanksref{Princeton}\nolinebreak,
%E.~Scapparone\thanksref{BOINFN}\nolinebreak,
%B.~Schlitzer\thanksref{UCDavis}\nolinebreak,
%G.~Scioli\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
%D.~A.~Semenov\thanksref{Petersburg}\nolinebreak,
%B.~Shaw\thanksref{TRIUMFaddress}\nolinebreak,
%A.~Shchagin\thanksref{Belgorod}\nolinebreak,
%A.~Sheshukov\thanksref{JINR}\nolinebreak,
%M.~Simeone\thanksref{NAUniCHE}{NAINFN}\nolinebreak,
%P.~Skensved\thanksref{Queens}\nolinebreak,
%M.~D.~Skorokhvatov\thanksref{Kurchatov}{MEPhI}\nolinebreak,
%O.~Smirnov\thanksref{JINR}\nolinebreak,
%B.~Smith\thanksref{TRIUMFaddress}\nolinebreak,
%A.~Sokolov\thanksref{BINP}{NSU}\nolinebreak,
R.~Stefanizzi\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
A.~Steri\thanksref{CAINFN}\nolinebreak,
%S.~Stracka\thanksref{PIINFN}\nolinebreak,
%V.~Strickland \thanksref{Carleton}\nolinebreak,
%M.~Stringer\thanksref{Queens}\nolinebreak,
S.~Sulis\thanksref{CAUniEEE}{CAINFN}\nolinebreak,
%Y.~Suvorov\thanksref{NAUniPHY}{NAINFN}{Kurchatov}\nolinebreak,
%A.~M.~Szelc\thanksref{Manchester}\nolinebreak,
%J.Z.~Szucs-Balazs\thanksref{INCDTIM}\nolinebreak,
R.~Tartaglia\thanksref{AQLNGS}\nolinebreak,
%G.~Testera\thanksref{GEINFN}\nolinebreak,
%T.~N.~Thorpe\thanksref{AQGSSI}{AQLNGS}\nolinebreak,
%A.~Tonazzo\thanksref{APC}\nolinebreak,
%S.~Torres-Lara\thanksref{Houston}\nolinebreak,
%.~Tosti\thanksref{ENEA}\nolinebreak,
%A.~Tricomi\thanksref{CTINFN}{CTUNI}\nolinebreak,
M.~Tuveri\thanksref{CAINFN}\nolinebreak,
%E.~V.~Unzhakov\thanksref{Petersburg}\nolinebreak,
%G.~Usai\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
%T.~Vallivilayil~John\thanksref{AQGSSI}{AQLNGS}\nolinebreak,
S.~Vescovi\thanksref{LNFINFN}\nolinebreak,
%T.~Viant\thanksref{ETHZ}\nolinebreak,
%S.~Viel\thanksref{Carleton}\nolinebreak,
%A.~Vishneva\thanksref{JINR}\nolinebreak,
%R.~B.~Vogelaar\thanksref{VTech}\nolinebreak,
M.~Wada\thanksref{AstroCeNT}\nolinebreak,
%H.~Wang\thanksref{UCLA}\nolinebreak,
%Y.~Wang\thanksref{UCLA}\nolinebreak,
%S.~Westerdale\thanksref{CAINFN}\nolinebreak,
%R.~J.~Wheadon\thanksref{TOINFN}\nolinebreak,
%L.~Williams\thanksref{FortLewis}\nolinebreak,
%Ma.~M.~Wojcik\thanksref{Krakow}\nolinebreak,
%Ma.~Wojcik\thanksref{Lodz}\nolinebreak,
%X.~Xiao\thanksref{UCLA}\nolinebreak,
%C.~Yang\thanksref{IHEPaddress}\nolinebreak,
A.~Zabihi\thanksref{AstroCeNT}\nolinebreak,

%A.~Zani\thanksref{CERNaddress}\nolinebreak,
%F.~Zenobio\thanksref{Polaris}\notds\nolinebreak,
%A.~Zichichi\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
%G.~Zuzel\thanksref{Krakow}\nolinebreak,
%M.~P.~Zykova\thanksref{MendeleevUniverisity}


%}

==> basic/author_list_end_2.tex <==

% \renewcommand{\thanksref}[1]{$^{\ref{#1}}$}
\newcommand{\notds}{\nolinebreak\footnotemark\nolinebreak}
\renewcommand{\thefootnote}{$*$}

{
\onecolumn
% \textbf{The Aria and DarkSide-20k Collaborations}
\textbf{The DarkSide-20k Collaboration}
\footnotetext{Not a member of the DarkSide-20k Collaboration}

% \newline
P.~Agnes\thanksref{Houston}\nolinebreak, 
S.~Albergo\thanksref{CTINFN}{CTUNI}\nolinebreak, 
I.~F.~M.~Albuquerque\thanksref{USP}\nolinebreak,
T.~Alexander\thanksref{PNNLaddress}\nolinebreak,
A.~Alici\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
A.~K.~Alton\thanksref{Augustana}\nolinebreak,
P.~Amaudruz\thanksref{TRIUMFaddress}\nolinebreak,
M.~Arba\thanksref{CAINFN}\nolinebreak,
P.~Arpaia\thanksref{NAUniPHY}\nolinebreak,
S.~Arcelli\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
M.~Ave\thanksref{USP}\nolinebreak,
 I.~Ch.~Avetissov\thanksref{MendeleevUniverisity}\nolinebreak,
R.~I.~Avetisov\thanksref{MendeleevUniverisity}\nolinebreak,
O.~Azzolini\thanksref{LNLINFN}\nolinebreak,
H.~O.~Back\thanksref{PNNLaddress}\nolinebreak,
Z.~Balmforth\thanksref{RHUL}\nolinebreak,
V.~Barbarian\thanksref{MSU}\nolinebreak,
A.~Barrado~Olmedo\thanksref{CIEMAT}\nolinebreak,
P.~Barrillon\thanksref{CPPM}\nolinebreak,
A.~Basco\thanksref{NAINFN}\nolinebreak,
G.~Batignani\thanksref{PIINFN}{PIUniPHY}\nolinebreak,
A.~Bondar\thanksref{BINP}{NSU}\nolinebreak,
W.~M.~Bonivento\thanksref{CAINFN}\nolinebreak,
E.~Borisova\thanksref{BINP}{NSU}\nolinebreak,
B.~Bottino\thanksref{GEUni}{GEINFN}\nolinebreak,
M.~G.~Boulay\thanksref{Carleton}\nolinebreak,
G.~Buccino\thanksref{CERNaddress}\nolinebreak,
S.~Bussino\thanksref{RMTreINFN}{RMTreUni}\nolinebreak,
J.~Busto\thanksref{CPPM}\nolinebreak,
A.~Buzulutskov\thanksref{BINP}{NSU}\nolinebreak,
M.~Cadeddu\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
M.~Cadoni\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
A.~Caminata\thanksref{GEINFN}\nolinebreak,
E.V.~Canesi\thanksref{Polaris}\notds\nolinebreak,
N.~Canci\thanksref{AQLNGS}\nolinebreak,
G.~Cappello\thanksref{CTINFN}{CTUNI}\nolinebreak,
M.~Caravati\thanksref{CAINFN}\nolinebreak,
M.~C\'ardenas-Montes\thanksref{CIEMAT}\nolinebreak,
N.~Cargioli\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
M.~Carlini\thanksref{AQGSSI}\nolinebreak,
F.~Carnesecchi\thanksref{BOINFN}{BOUniPHY}\nolinebreak,
P.~Castello\thanksref{CAUniEEE}{CAINFN}\nolinebreak,
A.~Castellani\thanksref{MIPoliICA}\nolinebreak,
S.~Catalanotti\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
V.~Cataudella\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
P.~Cavalcante\thanksref{AQLNGS}\nolinebreak,
S.~Cavuoti\thanksref{NAUniPHY}{NAINFN}{OACINAF}\nolinebreak,
S.~Cebrian\thanksref{Zaragoza}\nolinebreak,
J.~M.~Cela~Ruiz\thanksref{CIEMAT}\nolinebreak,
B.~Celano\thanksref{NAINFN}\nolinebreak,
S.~Chashin\thanksref{MSU}\nolinebreak,
A.~Chepurnov\thanksref{MSU}\nolinebreak,
C.~Cical\`o\thanksref{CAINFN}\nolinebreak,
L.~Cifarelli\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
D.~Cintas\thanksref{Zaragoza}\nolinebreak,
F.~Coccetti\thanksref{CentroFermi}\nolinebreak,
V.~Cocco\thanksref{CAINFN}\nolinebreak,
M.~Colocci\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
E.~Conde~Vilda\thanksref{CIEMAT}\nolinebreak,
L.~Consiglio\thanksref{AQLNGS}\nolinebreak,
S.~Copello\thanksref{GEINFN}{GEUni}\nolinebreak,
J.~Corning\thanksref{Queens}\nolinebreak,
G.~Covone\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
P.~Czudak\thanksref{Krakow}\nolinebreak,
M.~D'Aniello\thanksref{NAUniStruct}\nolinebreak,
S.~D'Auria\thanksref{MIINFN}\nolinebreak,
M.~D.~Da~Rocha~Rolo\thanksref{TOINFN}\nolinebreak,
O.~Dadoun\thanksref{LPNHE}\nolinebreak,
M.~Daniel\thanksref{CIEMAT}\nolinebreak,
S.~Davini\thanksref{GEINFN}\nolinebreak,
A.~De~Candia\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
S.~De~Cecco\thanksref{RMUnoINFN}{RMUnoUni}\nolinebreak,
A.~De~Falco\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
G.~De~Filippis\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
D.~De~Gruttola\thanksref{SAUni}{SAINFN}\nolinebreak,
G.~De~Guido\thanksref{MIPoliCHE}\nolinebreak,
G.~De~Rosa\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
M.~Della~Valle\thanksref{NAINFN}{OACINAF}\nolinebreak,
G.~Dellacasa\thanksref{TOINFN}\nolinebreak,
S.~De Pasquale\thanksref{SAUni}{SAINFN}\nolinebreak,
A.~V.~Derbin\thanksref{Petersburg}\nolinebreak,
A.~Devoto\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
L.~Di~Noto\thanksref{GEINFN}\nolinebreak,
F.~Di Eusanio\thanksref{Princeton}\nolinebreak,
C.~Dionisi\thanksref{RMUnoINFN}{RMUnoUni}\nolinebreak,
P.~Di Stefano\thanksref{Queens}\nolinebreak,
G.~Dolganov\thanksref{Kurchatov}\nolinebreak,
D.~Dongiovanni\thanksref{ENEA}\nolinebreak,
F.~Dordei\thanksref{CAINFN}\nolinebreak,
M.~Downing\thanksref{UMass}\nolinebreak,
T.~Erjavec\thanksref{UCDavis}\nolinebreak,
S.~Falciano\thanksref{AQGSSI}{RMUnoINFN}\nolinebreak,
S.~Farenzena\thanksref{CS}\notds\nolinebreak,
M.~Fernandez~Diaz\thanksref{CIEMAT}\nolinebreak,
C.~Filip\thanksref{INCDTIM}\nolinebreak,
G.~Fiorillo\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
A.~Franceschi\thanksref{LNFINFN}\nolinebreak,
D.~Franco\thanksref{APC}\nolinebreak,
E.~Frolov\thanksref{BINP}{NSU}\nolinebreak,
N.~Funicello\thanksref{SAUni}{SAINFN}\nolinebreak,
F.~Gabriele\thanksref{AQLNGS}\nolinebreak,
C.~Galbiati\thanksref{Princeton}{AQLNGS}{AQGSSI}\nolinebreak,
M.~Garbini\thanksref{CentroFermi}{BOINFN}\nolinebreak,
P.~Garcia~Abia\thanksref{CIEMAT}\nolinebreak,
A.~Gendotti\thanksref{ETHZ}\nolinebreak,
C.~Ghiano\thanksref{AQLNGS}\nolinebreak,
R.~A.~Giampaolo\thanksref{TOINFN}{TOPoli}\nolinebreak,
C.~Giganti\thanksref{LPNHE}\nolinebreak,
M.~A.~Giorgi\thanksref{PIUniPHY}{PIINFN}\nolinebreak,
G.~K.~Giovanetti\thanksref{WilliamsCollege}\nolinebreak,
M.L.~Gligan\thanksref{INCDTIM}\nolinebreak,
V.~Goicoechea~Casanueva\thanksref{Hawaii}\nolinebreak,
A.~Gola\thanksref{TNFBK}{TNTIFPA}\nolinebreak,
A.M.~Goretti\thanksref{AQLNGS}\nolinebreak,
R.~Graciani~Diaz\thanksref{UB}\nolinebreak,
G.~Y.~Grigoriev\thanksref{Kurchatov}\nolinebreak,
A.~Grobov\thanksref{Kurchatov}{MEPhI}\nolinebreak,
M.~Gromov\thanksref{MSU}{JINR}\nolinebreak,
M.~Guan\thanksref{IHEPaddress}\nolinebreak,
M.~Guerzoni\thanksref{BOINFN}\nolinebreak,
M.~Guetti\thanksref{AQLNGS}\nolinebreak,
M.~Gulino\thanksref{ENUniCEE}{CTLNS}\nolinebreak,
C.~Guo\thanksref{IHEPaddress}\nolinebreak,
B.~R.~Hackett\thanksref{PNNLaddress}\nolinebreak,
A.~Hallin\thanksref{Alberta}\nolinebreak,
M.~Haranczyk\thanksref{Krakow}\nolinebreak,
S.~Hill\thanksref{RHUL}\nolinebreak,
S.~Horikawa\thanksref{AQGSSI}{AQLNGS}\nolinebreak,
F.~Hubaut\thanksref{CPPM}\nolinebreak,
T.~Hugues\thanksref{AstroCeNT}\nolinebreak,
E.~V.~Hungerford\thanksref{Houston}\nolinebreak,
An.~Ianni\thanksref{Princeton}{AQLNGS}\nolinebreak,
V.~Ippolito\thanksref{RMUnoINFN}\nolinebreak,
C.~C.~James\thanksref{FNALaddress}\nolinebreak,
C.~Jillings\thanksref{SNOLABaddress}{Laurentian}\nolinebreak,
P.~Kachru\thanksref{AQGSSI}{AQLNGS}\nolinebreak,
A.~A.~Kemp\thanksref{Queens}\nolinebreak,
C.~L.~Kendziora\thanksref{FNALaddress}\nolinebreak,
G.~Keppel\thanksref{LNLINFN}\nolinebreak,
A.~V.~Khomyakov\thanksref{MendeleevUniverisity}\nolinebreak,
% S.~Kim\thanksref{Temple}\nolinebreak,
A.~Kish\thanksref{Hawaii}\nolinebreak,
I.~Kochanek\thanksref{AQLNGS}\nolinebreak,
K.~Kondo\thanksref{AQLNGS}\nolinebreak,
G.~Korga\thanksref{RHUL}\nolinebreak,
A.~Kubankin\thanksref{Belgorod}\nolinebreak,
R.~Kugathasan\thanksref{TOINFN}{TOPoli}\nolinebreak,
M.~Kuss\thanksref{PIINFN}\nolinebreak,
M.~Kuźniak\thanksref{AstroCeNT}\nolinebreak,
M.~La~Commara\thanksref{NAUniPHARM}{NAINFN}\nolinebreak,
L.~La Delfa\thanksref{CAINFN}\nolinebreak,
D.~La Grasta\thanksref{Polaris}\notds\nolinebreak,
M.~Lai\thanksref{CAUniPHY}{CAINFN}{APC}\nolinebreak,
N.~Lami\thanksref{CS}\notds\nolinebreak,
S.~Langrock\thanksref{Laurentian}\nolinebreak,
M.~Leyton\thanksref{NAINFN}\nolinebreak,
X.~Li\thanksref{Princeton}\nolinebreak,
L.~Lidey\thanksref{PNNLaddress}\nolinebreak,
F.~Lippi\thanksref{CS}\notds\nolinebreak,
M.~Lissia\thanksref{CAINFN}\nolinebreak,
G.~Longo\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
N.~Maccioni\thanksref{CS}\notds\nolinebreak,
I.~N.~Machulin\thanksref{Kurchatov}{MEPhI}\nolinebreak,
L.~Mapelli\thanksref{Princeton}\nolinebreak,
A.~Marasciulli\thanksref{PIUniPHY}\nolinebreak,
A.~Margotti\thanksref{BOINFN}\nolinebreak,
S.~M.~Mari\thanksref{RMTreINFN}{RMTreUni}\nolinebreak,
J.~Maricic\thanksref{Hawaii}\nolinebreak,
M.~Marinelli\thanksref{GEINFN}\nolinebreak,
M.~Mart\'inez\thanksref{Zaragoza}{ZaragozaARAID}\nolinebreak,
A.~D.~Martinez~Rojas\thanksref{TOINFN}{TOPoli}\nolinebreak,
A.~Martini\thanksref{CS}{MISE}\notds\nolinebreak,
% C.~J.~Martoff\thanksref{Temple}\nolinebreak,
M.~Mascia\thanksref{CAUniCHE}\nolinebreak,
M.~Masetto\thanksref{Polaris}\notds\nolinebreak,
A.~Masoni\thanksref{CAINFN}\nolinebreak,
A.~Mazzi\thanksref{TNFBK}{TNTIFPA}\nolinebreak,
A.~B.~McDonald\thanksref{Queens}\nolinebreak,
J.~Mclaughlin\thanksref{TRIUMFaddress}{RHUL}\nolinebreak,
A.~Messina\thanksref{RMUnoINFN}{RMUnoUni}\nolinebreak,
P.~D.~Meyers\thanksref{Princeton}\nolinebreak,
T.~Miletic\thanksref{Hawaii}\nolinebreak,
R.~Milincic\thanksref{Hawaii}\nolinebreak,
R.~Miola\thanksref{Polaris}\notds\nolinebreak,
A.~Moggi\thanksref{PIINFN}\nolinebreak,
A.~Moharana\thanksref{AQGSSI}{AQLNGS}\nolinebreak,
S.~Moioli\thanksref{MIPoliCHE}\nolinebreak,
J.~Monroe\thanksref{RHUL}\nolinebreak,
S.~Morisi\thanksref{NAUniPHY}{NAINFN}\nolinebreak,
M.~Morrocchi\thanksref{PIINFN}{PIUniPHY}\nolinebreak,
E.~N.~Mozhevitina\thanksref{MendeleevUniverisity}\nolinebreak,
T.~Mr\'oz\thanksref{Krakow}\nolinebreak,
V.~N.~Muratova\thanksref{Petersburg}\nolinebreak,
A.~Murenu\thanksref{CAINFN}\nolinebreak,
C.~Muscas\thanksref{CAUniEEE}{CAINFN}\nolinebreak,
L.~Musenich\thanksref{GEINFN}{GEUni}\nolinebreak,
P.~Musico\thanksref{GEINFN}\nolinebreak,
R.~Nania\thanksref{BOINFN}\nolinebreak,
T.~Napolitano\thanksref{LNFINFN}\nolinebreak,
A.~Navrer~Agasson\thanksref{LPNHE}\nolinebreak,
M.~Nessi\thanksref{CERNaddress}\nolinebreak,
I.~Nikulin\thanksref{Belgorod}\nolinebreak,
J.~Nowak\thanksref{Lancaster}\nolinebreak,
A.~Oleinik\thanksref{Belgorod}\nolinebreak,
V.~Oleynikov\thanksref{BINP}{NSU}\nolinebreak,
L.~Pagani\thanksref{UCDavis}\nolinebreak,
M.~Pallavicini\thanksref{GEUni}{GEINFN}\nolinebreak,
S.~Palmas\thanksref{CAUniCHE}\nolinebreak,
L.~Pandola\thanksref{CTLNS}\nolinebreak,
E.~Pantic\thanksref{UCDavis}\nolinebreak,
E.~Paoloni\thanksref{PIINFN}{PIUniPHY}\nolinebreak,
G.~Paternoster\thanksref{TNFBK}{TNTIFPA}\nolinebreak,
P.~A.~Pegoraro\thanksref{CAUniEEE}{CAINFN}\nolinebreak,
L.~A.~Pellegrini\thanksref{MIPoliCHE}\nolinebreak,
C.~Pellegrino\thanksref{BOINFN}\nolinebreak,
K.~Pelczar\thanksref{Krakow}\nolinebreak,
F.~Perotti\thanksref{MIPoliICA}{MIINFN}\nolinebreak,
V.~Pesudo\thanksref{CIEMAT}\nolinebreak,
E.~Picciau\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
F.~Pietropaolo\thanksref{CERNaddress}\nolinebreak,
T.~Pinna\thanksref{ENEA}\nolinebreak,
A.~Pocar\thanksref{UMass}\nolinebreak,
P.~Podda\thanksref{CS}\notds\nolinebreak,
D.~M.~Poehlmann\thanksref{UCDavis}\nolinebreak,
S.~Pordes\thanksref{FNALaddress}\nolinebreak,
S.~S.~Poudel\thanksref{Houston}\nolinebreak,
P.~Pralavorio\thanksref{CPPM}\nolinebreak,
D.~Price\thanksref{Manchester}\nolinebreak,
F.~Raffaelli\thanksref{PIINFN}\nolinebreak,
F.~Ragusa\thanksref{MIUni}{MIINFN}\nolinebreak,
A.~Ramirez\thanksref{Houston}\nolinebreak,
M.~Razeti\thanksref{CAINFN}\nolinebreak,
A.~Razeto\thanksref{AQLNGS}\nolinebreak,
A.~L.~Renshaw\thanksref{Houston}\nolinebreak,
S.~Rescia\thanksref{BNLaddress}\nolinebreak,
M.~Rescigno\thanksref{RMUnoINFN}\nolinebreak,
F.~Resnati\thanksref{CERNaddress}\nolinebreak,
F.~Retiere\thanksref{TRIUMFaddress}\nolinebreak,
L.~P.~Rignanese\thanksref{BOINFN}{BOUniPHY}\nolinebreak,
C.~Ripoli\thanksref{SAINFN}{SAUni}\nolinebreak,
A.~Rivetti\thanksref{TOINFN}\nolinebreak,
J.~Rode\thanksref{LPNHE}{APC}\nolinebreak,
L.~Romero\thanksref{CIEMAT}\nolinebreak,
M.~Rossi\thanksref{GEINFN}{GEUni}\nolinebreak,
A.~Rubbia\thanksref{ETHZ}\nolinebreak,
M.~Rucaj\thanksref{Polaris}\notds\nolinebreak,
G.M.~Sabiu\thanksref{CS}\notds\nolinebreak,
P.~Salatino\thanksref{NAUniCHE}{NAINFN}\nolinebreak,
O.~Samoylov\thanksref{JINR}\nolinebreak,
E.~S\'anchez~Garc\'ia\thanksref{CIEMAT}\nolinebreak,
E.~Sandford\thanksref{Manchester}\nolinebreak,
S.~Sanfilippo\thanksref{RMTreUni}{RMTreINFN}\nolinebreak,
V.A.~Sangiorgio\thanksref{MIPoliCHE}\nolinebreak,
V.~Santacroce\thanksref{CS}\notds\nolinebreak,
D.~Santone\thanksref{RHUL}\nolinebreak,
R.~Santorelli\thanksref{CIEMAT}\nolinebreak,
A.~Santucci\thanksref{ENEA}\nolinebreak,
C.~Savarese\thanksref{Princeton}\nolinebreak,
E.~Scapparone\thanksref{BOINFN}\nolinebreak,
B.~Schlitzer\thanksref{UCDavis}\nolinebreak,
G.~Scioli\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
D.~A.~Semenov\thanksref{Petersburg}\nolinebreak,
B.~Shaw\thanksref{TRIUMFaddress}\nolinebreak,
A.~Shchagin\thanksref{Belgorod}\nolinebreak,
A.~Sheshukov\thanksref{JINR}\nolinebreak,
M.~Simeone\thanksref{NAUniCHE}{NAINFN}\nolinebreak,
P.~Skensved\thanksref{Queens}\nolinebreak,
M.~D.~Skorokhvatov\thanksref{Kurchatov}{MEPhI}\nolinebreak,
O.~Smirnov\thanksref{JINR}\nolinebreak,
B.~Smith\thanksref{TRIUMFaddress}\nolinebreak,
A.~Sokolov\thanksref{BINP}{NSU}\nolinebreak,
R.~Stefanizzi\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
A.~Steri\thanksref{CAINFN}\nolinebreak,
S.~Stracka\thanksref{PIINFN}\nolinebreak,
V.~Strickland \thanksref{Carleton}\nolinebreak,
M.~Stringer\thanksref{Queens}\nolinebreak,
S.~Sulis\thanksref{CAUniEEE}{CAINFN}\nolinebreak,
Y.~Suvorov\thanksref{NAUniPHY}{NAINFN}{Kurchatov}\nolinebreak,
A.~M.~Szelc\thanksref{Manchester}\nolinebreak,
J.Z.~Szucs-Balazs\thanksref{INCDTIM}\nolinebreak,
R.~Tartaglia\thanksref{AQLNGS}\nolinebreak,
G.~Testera\thanksref{GEINFN}\nolinebreak,
T.~N.~Thorpe\thanksref{AQGSSI}{AQLNGS}\nolinebreak,
A.~Tonazzo\thanksref{APC}\nolinebreak,
S.~Torres-Lara\thanksref{Houston}\nolinebreak,
S.~Tosti\thanksref{ENEA}\nolinebreak,
A.~Tricomi\thanksref{CTINFN}{CTUNI}\nolinebreak,
M.~Tuveri\thanksref{CAINFN}\nolinebreak,
E.~V.~Unzhakov\thanksref{Petersburg}\nolinebreak,
G.~Usai\thanksref{CAUniPHY}{CAINFN}\nolinebreak,
T.~Vallivilayil~John\thanksref{AQGSSI}{AQLNGS}\nolinebreak,
S.~Vescovi\thanksref{LNFINFN}\nolinebreak,
T.~Viant\thanksref{ETHZ}\nolinebreak,
S.~Viel\thanksref{Carleton}\nolinebreak,
A.~Vishneva\thanksref{JINR}\nolinebreak,
R.~B.~Vogelaar\thanksref{VTech}\nolinebreak,
M.~Wada\thanksref{AstroCeNT}\nolinebreak,
H.~Wang\thanksref{UCLA}\nolinebreak,
Y.~Wang\thanksref{UCLA}\nolinebreak,
S.~Westerdale\thanksref{CAINFN}\nolinebreak,
R.~J.~Wheadon\thanksref{TOINFN}\nolinebreak,
L.~Williams\thanksref{FortLewis}\nolinebreak,
Ma.~M.~Wojcik\thanksref{Krakow}\nolinebreak,
Ma.~Wojcik\thanksref{Lodz}\nolinebreak,
X.~Xiao\thanksref{UCLA}\nolinebreak,
C.~Yang\thanksref{IHEPaddress}\nolinebreak,
A.~Zani\thanksref{CERNaddress}\nolinebreak,
F.~Zenobio\thanksref{Polaris}\notds\nolinebreak,
A.~Zichichi\thanksref{BOUniPHY}{BOINFN}\nolinebreak,
G.~Zuzel\thanksref{Krakow}\nolinebreak,
M.~P.~Zykova\thanksref{MendeleevUniverisity}

\begin{enumerate}[label=\textsuperscript{\arabic*}]
    \item {\label{Houston}\Houston}
    \item {\CTINFN \label{CTINFN}}
    \item {\CTUNI \label{CTUNI}}
    \item {\USP \label{USP}}
    \item {\PNNLaddress \label{PNNLaddress}}
    \item {\BOUniPHY \label{BOUniPHY}}
    \item {\BOINFN \label{BOINFN}}
    \item {\Augustana \label{Augustana}}
    \item {\TRIUMFaddress \label{TRIUMFaddress}}
    \item {\MendeleevUniverisity \label{MendeleevUniverisity}}
    \item {\LNLINFN \label{LNLINFN}}
    \item {\RHUL \label{RHUL}}
    \item {\MSU \label{MSU}}
    \item {\CIEMAT \label{CIEMAT}}
    \item {\CPPM \label{CPPM}}
    \item {\NAINFN \label{NAINFN}}
    \item {\PIINFN \label{PIINFN}}
    \item {\PIUniPHY \label{PIUniPHY}}
    \item {\BINP \label{BINP}}
    \item {\NSU \label{NSU}}
    \item {\CAINFN \label{CAINFN}}
    \item {\GEUni \label{GEUni}}
    \item {\GEINFN \label{GEINFN}}
    \item {\Carleton \label{Carleton}}
    \item {\CERNaddress \label{CERNaddress}}
    \item {\RMTreINFN \label{RMTreINFN}}
    \item {\RMTreUni \label{RMTreUni}}
    \item {\CAUniPHY \label{CAUniPHY}}
    \item {\AQLNGS \label{AQLNGS}}
    \item {\AQGSSI \label{AQGSSI}}
    \item {\CentroFermi \label{CentroFermi}}
    \item {\CAUniEEE \label{CAUniEEE}}
    \item {\NAUniPHY \label{NAUniPHY}}
    \item {\NAUniStruct \label{NAUniStruct}}
    \item {\OACINAF \label{OACINAF}}
    \item {\Zaragoza \label{Zaragoza}}
    \item {\Krakow \label{Krakow}}
    \item {\MIINFN \label{MIINFN}}
    \item {\TOINFN \label{TOINFN}}
    \item {\LPNHE \label{LPNHE}}
    \item {\RMUnoINFN \label{RMUnoINFN}}
    \item {\RMUnoUni \label{RMUnoUni}}
    \item {\SAUni \label{SAUni}}
    \item {\SAINFN \label{SAINFN}}
    \item {\MIPoliCHE \label{MIPoliCHE}}
    \item {\Petersburg \label{Petersburg}}
    \item {\Kurchatov \label{Kurchatov}}
    \item {\UMass \label{UMass}}
    \item {\UCDavis \label{UCDavis}}
    \item {\LNFINFN \label{LNFINFN}}
    \item {\APC \label{APC}}
    \item {\Princeton \label{Princeton}}
    \item {\ETHZ \label{ETHZ}}
    \item {\TOPoli \label{TOPoli}}
    \item {\WilliamsCollege \label{WilliamsCollege}}
    \item {\Hawaii \label{Hawaii}}
    \item {\TNFBK \label{TNFBK}}
    \item {\TNTIFPA \label{TNTIFPA}}
    \item {\UB \label{UB}}
    \item {\MEPhI \label{MEPhI}}
    \item {\JINR \label{JINR}}
    \item {\IHEPaddress \label{IHEPaddress}}
    \item {\ENUniCEE \label{ENUniCEE}}
    \item {\CTLNS \label{CTLNS}}
    \item {\Alberta \label{Alberta}}
    \item {\AstroCeNT \label{AstroCeNT}}
    \item {\FNALaddress \label{FNALaddress}}
    \item {\SNOLABaddress \label{SNOLABaddress}}
    \item {\Laurentian \label{Laurentian}}
    % \item {\Temple \label{Temple}}
    \item {\Belgorod \label{Belgorod}}
    \item {\NAUniPHARM \label{NAUniPHARM}}
    \item {\ZaragozaARAID \label{ZaragozaARAID}}
    \item {\Queens \label{Queens}}
    \item {\Lancaster \label{Lancaster}}
    \item {\MIPoliICA \label{MIPoliICA}}
    \item {\Manchester \label{Manchester}}
    \item {\MIUni \label{MIUni}}
    \item {\BNLaddress \label{BNLaddress}}
    \item {\NAUniCHE \label{NAUniCHE}}
    \item {\VTech \label{VTech}}
    \item {\UCLA \label{UCLA}}
    \item {\FortLewis \label{FortLewis}}
    \item {\Lodz \label{Lodz}}
    \item {\CAUniCHE \label{CAUniCHE}}
    \item {\INCDTIM \label{INCDTIM}}
    \item {\ENEA \label{ENEA}}
    \item {\CS \label{CS}}
    \item {\Polaris \label{Polaris}}
    \item {\MISE \label{MISE}}
\end{enumerate}
}

==> basic/inst.tex <==
\newcommand{\Alberta}{Department of Physics, University of Alberta, Edmonton, AB T6G 2R3, Canada}
\newcommand{\APC}{APC, Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, Paris F-75013, France}
\newcommand{\AQLNGS}{INFN Laboratori Nazionali del Gran Sasso, Assergi (AQ) 67100, Italy}
\newcommand{\AQGSSI}{Gran Sasso Science Institute, L'Aquila 67100, Italy}
\newcommand{\AQUni}{Università degli Studi dell'Aquila, L'Aquila 67100, Italy}
\newcommand{\AstroCeNT}{AstroCeNT, Nicolaus Copernicus Astronomical Center of the Polish Academy of Sciences, 00-614 Warsaw, Poland}
\newcommand{\Augustana}{Physics Department, Augustana University, Sioux Falls, SD 57197, USA}
\newcommand{\Belgorod}{Radiation Physics Laboratory, Belgorod National Research University, Belgorod 308007, Russia}
\newcommand{\BHSU}{School of Natural Sciences, Black Hills State University, Spearfish, SD 57799, USA}
\newcommand{\BINP}{Budker Institute of Nuclear Physics, Novosibirsk 630090, Russia}
\newcommand{\BNLaddress}{Brookhaven National Laboratory, Upton, NY 11973, USA}
\newcommand{\BOINFN}{INFN Bologna, Bologna 40126, Italy}
\newcommand{\BOUniPHY}{Physics Department, Universit\`a degli Studi di Bologna, Bologna 40126, Italy}
\newcommand{\CS}{CarboSulcis S.p.A. - Miniera Monte Sinni, Cortoghiana 09010, Italy}
\newcommand{\CAUniCHE}{Department of Mechanical, Chemical, and Materials Engineering, Universit\`a degli Studi, Cagliari 09123, Italy}
\newcommand{\CAUniEEE}{Department of Electrical and Electronic Engineering, Universit\`a degli Studi di Cagliari, Cagliari 09123, Italy}
\newcommand{\CAUniPHY}{Physics Department, Universit\`a degli Studi di Cagliari, Cagliari 09042, Italy}
\newcommand{\CAINFN}{INFN Cagliari, Cagliari 09042, Italy}
\newcommand{\Carleton}{Department of Physics, Carleton University, Ottawa, ON K1S 5B6, Canada}
\newcommand{\Campinas}{Physics Institute, Universidade Estadual de Campinas, Campinas 13083, Brazil}
\newcommand{\Columbia}{Physics Department, Columbia University, New York, NY 10027, USA}
\newcommand{\Chicago}{Department of Physics and Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\newcommand{\CentroFermi}{Museo della fisica e Centro studi e Ricerche Enrico Fermi, Roma 00184, Italy}
\newcommand{\CERNaddress}{CERN, European Organization for Nuclear Research 1211 Geneve 23, Switzerland, CERN}
\newcommand{\CIEMAT}{CIEMAT, Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas, Madrid 28040, Spain}
\newcommand{\Cluj}{National Institute for R\&D of Isotopic and Molecular Technologies, Cluj-Napoca, 400293, Romania}
\newcommand{\CPPM}{Centre de Physique des Particules de Marseille, Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}
\newcommand{\CTINFN}{INFN Catania, Catania 95121, Italy}
\newcommand{\CTUNI}{Universit\`a of Catania, Catania 95124, Italy}
\newcommand{\CTLNS}{INFN Laboratori Nazionali del Sud, Catania 95123, Italy}
\newcommand{\ENEA}{Department of Fusion and Nuclear Safety Technologies, ENEA, Frascati 00044, Italy} 
\newcommand{\ENUniCEE}{Engineering and Architecture Faculty, Universit\`a di Enna Kore, Enna 94100, Italy}
\newcommand{\ETHZ}{Institute for Particle Physics, ETH Z\"urich, Z\"urich 8093, Switzerland}
\newcommand{\FNALaddress}{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
\newcommand{\FortLewis}{Department of Physics and Engineering, Fort Lewis College, Durango, CO 81301, USA}
\newcommand{\GEUni}{Physics Department, Universit\`a degli Studi di Genova, Genova 16146, Italy}
\newcommand{\GEINFN}{INFN Genova, Genova 16146, Italy}
\newcommand{\Hawaii}{Department of Physics and Astronomy, University of Hawai'i, Honolulu, HI 96822, USA}
\newcommand{\Houston}{Department of Physics, University of Houston, Houston, TX 77204, USA}
\newcommand{\IHEPaddress}{Institute of High Energy Physics, Beijing 100049, China}
\newcommand{\INCDTIM}{National Institute for Research and Development of Isotope and Molecular Technologies, Cluj-Napoca 400293,
Romania}
\newcommand{\IPNO}{Institut de Physique Nucl\`eaire d'Orsay, 91406, Orsay, France}
\newcommand{\INSTM}{Interuniversity Consortium for Science and Technology of Materials, Firenze 50121, Italy}
\newcommand{\IPHC}{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, Strasbourg 67037, France}
\newcommand{\JINR}{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\newcommand{\Krakow}{M.~Smoluchowski Institute of Physics, Jagiellonian University, 30-348 Krakow, Poland}
\newcommand{\Kurchatov}{National Research Centre Kurchatov Institute, Moscow 123182, Russia}
\newcommand{\Laurentian}{Department of Physics and Astronomy, Laurentian University, Sudbury, ON P3E 2C6, Canada}
\newcommand{\Lancaster}{Physics Department, Lancaster University, Lancaster LA1 4YB, UK}
\newcommand{\LNFINFN}{INFN Laboratori Nazionali di Frascati, Frascati 00044, Italy}
\newcommand{\LNLINFN}{INFN Laboratori Nazionali di Legnaro, Legnaro (Padova) 35020, Italy}
\newcommand{\Lodz}{Institute of Applied Radiation Chemistry, Lodz University of Technology, 93-590 Lodz, Poland}
\newcommand{\LPNHE}{LPNHE, CNRS/IN2P3, Sorbonne Universit\'e, Universit\'e Paris Diderot, Paris 75252, France}
\newcommand{\Mainz}{Institut f\"ur Physik, Johannes Gutenberg-UniversitÃ€t Mainz, Mainz 55099, Germany}
\newcommand{\Manchester}{Department of Physics and Astronomy, The University of Manchester, Manchester M13 9PL, UK}
\newcommand{\MEPhI}{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\newcommand{\MendeleevUniverisity}{Mendeleev University of Chemical Technology, Moscow 125047, Russia}
\newcommand{\MIBIINFN}{INFN Milano Bicocca, Milano 20126, Italy}
\newcommand{\MIINFN}{INFN Milano, Milano 20133, Italy}
\newcommand{\MIPoliICA}{Civil and Environmental Engineering Department, Politecnico di Milano, Milano 20133, Italy}
\newcommand{\MIPoliCHE}{Chemistry, Materials and Chemical Engineering Department ``G.~Natta", Politecnico di Milano, Milano 20133, Italy}
\newcommand{\MIPoliEIB}{Electronics, Information, and Bioengineering Department, Politecnico di Milano, Milano 20133, Italy}
\newcommand{\MIPoliENE}{Energy Department, Politecnico di Milano, Milano 20133, Italy}
\newcommand{\MIUni}{Physics Department, Universit\`a degli Studi di Milano, Milano 20133, Italy}
\newcommand{\MSU}{Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Moscow 119234, Russia}
\newcommand{\NAINFN}{INFN Napoli, Napoli 80126, Italy}
\newcommand{\NAUniPHY}{Physics Department, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80126, Italy}
\newcommand{\NAUniCHE}{Chemical, Materials, and Industrial Production Engineering Department, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80126, Italy}
\newcommand{\NAUniPHARM}{Pharmacy Department, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80131, Italy}
\newcommand{\NAUniStruct}{Dipartimento di Strutture per l'Ingegneria e l'Architettura, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80131, Italy}
\newcommand{\NAUniEEIT}{Department of Electrical Engineering and Information Technology, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80125, Italy}
\newcommand{\NSU}{Novosibirsk State University, Novosibirsk 630090, Russia}
\newcommand{\OACINAF}{INAF Osservatorio Astronomico di Capodimonte, 80131 Napoli, Italy}
\newcommand{\Petersburg}{Saint Petersburg Nuclear Physics Institute, Gatchina 188350, Russia}
\newcommand{\PGUniCBB}{Chemistry, Biology and Biotechnology Department, Universit\`a degli Studi di Perugia, Perugia 06123, Italy}
\newcommand{\PGINFN}{INFN Perugia, Perugia 06123, Italy}
\newcommand{\PIINFN}{INFN Pisa, Pisa 56127, Italy}
\newcommand{\PIUniPHY}{Physics Department, Universit\`a degli Studi di Pisa, Pisa 56127, Italy}
\newcommand{\PNNLaddress}{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\newcommand{\Princeton}{Physics Department, Princeton University, Princeton, NJ 08544, USA}
\newcommand{\Polaris}{Polaris S.r.l., Misinto 20826, Italy}
\newcommand{\Queens}{Department of Physics, Engineering Physics and Astronomy, Queen's University, Kingston, ON K7L 3N6, Canada}
\newcommand{\RHUL}{Department of Physics, Royal Holloway University of London, Egham TW20 0EX, UK}
\newcommand{\RMTreINFN}{INFN Roma Tre, Roma 00146, Italy}
\newcommand{\RMTreUni}{Mathematics and Physics Department, Universit\`a degli Studi Roma Tre, Roma 00146, Italy}
\newcommand{\RMUnoINFN}{INFN Sezione di Roma, Roma 00185, Italy}
\newcommand{\RMUnoUni}{Physics Department, Sapienza Universit\`a di Roma, Roma 00185, Italy}
\newcommand{\SAINFN}{INFN Salerno, Salerno 84084, Italy}
\newcommand{\SAUni}{Physics Department, Universit\`a degli Studi di Salerno, Salerno 84084, Italy}
\newcommand{\SNOLABaddress}{SNOLAB, Lively, ON P3Y 1N2, Canada}
\newcommand{\SSUniCHP}{Chemistry and Pharmacy Department, Universit\`a degli Studi di Sassari, Sassari 07100, Italy}
\newcommand{\Sussex}{Physics and Astronomy Department, University of Sussex, Brighton BN1 9QH, UK}
\newcommand{\Temple}{Physics Department, Temple University, Philadelphia, PA 19122, USA}
\newcommand{\TNFBK}{Fondazione Bruno Kessler, Povo 38123, Italy}
\newcommand{\TNTIFPA}{Trento Institute for Fundamental Physics and Applications, Povo 38123, Italy}
\newcommand{\TNUni}{Physics Department, Universit\`a degli Studi di Trento, Povo 38123, Italy}
\newcommand{\TOINFN}{INFN Torino, Torino 10125, Italy}
\newcommand{\TOPoli}{Department of Electronics and Communications, Politecnico di Torino, Torino 10129, Italy}
\newcommand{\TOUni}{Physics Department, Universit\`a degli Studi di Torino, Torino 10125, Italy}
\newcommand{\TRIUMFaddress}{TRIUMF, 4004 Wesbrook Mall, Vancouver, BC V6T 2A3, Canada}
\newcommand{\TUM}{Physik Department, Technische Universit\"at M\"unchen, Munich 80333, Germany}
\newcommand{\UB}{Universiatat de Barcelona, Barcelona E-08028, Catalonia, Spain} 
\newcommand{\UCDavis}{Department of Physics, University of California, Davis, CA 95616, USA}
\newcommand{\UCSanDiego}{Department of Physics, University of California, San Diego, CA 92093, USA}
\newcommand{\UCLA}{Physics and Astronomy Department, University of California, Los Angeles, CA 90095, USA}
\newcommand{\UMass}{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\newcommand{\UNAM}{Instituto de F\'isica, Universidad Nacional Aut\'onoma de M\'exico, M\'exico 01000, Mexico}
\newcommand{\UOC}{Department of Chemistry, University of Crete, P.O. Box 2208, 71003 Heraklion, Crete, Greece}
\newcommand{\USP}{Instituto de F\'isica, Universidade de S\~ao Paulo, S\~ao Paulo 05508-090, Brazil}
\newcommand{\VTech}{Virginia Tech, Blacksburg, VA 24061, USA}
\newcommand{\WilliamsCollege}{Williams College, Physics Department, Williamstown, MA 01267 USA}
\newcommand{\Zaragoza}{Centro de Astropart\'iculas y F\'isica de Altas Energ\'ias, Universidad de Zaragoza, Zaragoza 50009, Spain}
\newcommand{\ZaragozaARAID}{Fundaci\'on ARAID, Universidad de Zaragoza, Zaragoza 50009, Spain}
\newcommand{\MISE}{Now at Ministero dello Sviluppo Economico, Palazzo Piacentini,
00187 Roma, Italy}

==> sections/asymmetry.tex <==
\section{Distillation asymmetry}
\label{sec:asy}
%Separation (between \ce{^36Ar} and \ce{^40Ar}) is given by 
As in Eq. \ref{frazione}, we define the 
%, that is the ratio between the lighter and the heavier element at the top divided by the same quantity distilled from the bottom of the column.\\
%Furthermore, 
 separation between top and feed, and between feed and bottom as:

\begin{equation} \label{TF} S^{TF}_{36-40}=\frac{{\left(\frac{x_{36}}{{x_{40}}}\right)_T}}{{\left(\frac{{x_{36}}}{{x_{40}}}\right)_F} }, \end{equation}

\begin{equation} \label{FB} S^{FB}_{36-40}=\frac{{\left(\frac{x_{36}}{{x_{40}}}\right)_F}}{{\left(\frac{{x_{36}}}{{x_{40}}}\right)_B} }, \end{equation}

%where the concentration of argon at the feed is expected to correspond to the natural abundances. 
%However, due to the variation of pressure occurred during the run, the measurement of the ${x_{36}}/{x_{40}}$ performed with the UGA is not reliable and only the ratio of this quantity at two different conditions (for instance at the top and bottom of the column) could be taken into account
As a matter of fact:

\begin{equation}S^{TB}_{36-40}=S^{TF}_{36-40} \times S^{FB}_{36-40},\end{equation}

We note from Fig.\ref{Setup23} that the isotope enrichment and depletion  are not symmetric. Fig \ref{ass2} shows the two separations defined in  Eq. \ref{TF} and Eq.\ref{FB} vs time. The time averaged values are reported in Table \ref{tab_sep}. 


%we, therefore, note how the overall separation is due to two components, one concerning the enrichment of the light element in the upper part of the column and the other which instead quantifies its decrease in the lower part. It is thus possible that the separation made by the column is asymmetrical concerning the top or bottom or that one of the two aforementioned separations has a greater weight than the other on the overall separation.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{images/ass_tutti.pdf}
\caption{Separation between \ce{^36Ar} and \ce{^40Ar} as function of time (hours) of the run. In red is the separation between top and feed of column (Eq. \ref{TF}) and in blue the one between feed and bottom (Eq. \ref{FB}). The grayed regions  correspond to   changing conditions in the column (see Fig. \ref{totalissimo}) and are not included in  the data analysis. }
\label{ass2}
\end{figure}

\begin{table}
%\setlength{\tabcolsep}{pt}
\setlength{\tabcolsep}{34pt}
\centering
\caption{Time averaged separation ${\cal S}^{TB}_{36-40}$ and $S^{BF}_{36-40}$  for runs A, B, and C. }
\begin{tabular}{@{} l l l @{}}
\hline\noalign{\smallskip}
& ${\cal S}^{TF}_{36-40}$ &${\cal S}^{FB}_{36-40}$ \\
\noalign{\smallskip}\hline\noalign{\smallskip}
A&$1.360  \pm0.003 $&$1.086  \pm0.009$\\ 
B&$1.366  \pm 0.003 $&$1.099  \pm0.008$\\ 
C&$1.331 \pm 0.002 $&$1.105  \pm0.005$\\ 
\hline
\end{tabular}
\label{tab_sep}
\end{table}


As can been seen from Fig. \ref{ass2} and in table \ref{tab_sep}, the separation between top and feed is about 30\%  larger than between feed and bottom. 
%This indicates how the enrichment of \ce{^36Ar} at the top of the column is always greater than its depletion at the bottom of it. 
This effect is possibly due to the stagnation of the less volatile isotope, \ce{^40Ar}, at the bottom of the column. If this were indeed the cause, we would expect a strong dependence of this asymmetry on the vapor mass flow rate inside the column.
%, since  a larger flow is expected to mix the isotopes in the column and therefore reduce the asymmetry. 
This expectation is confirmed by both the data and the simulation, whose results are displayed together in 
Fig. \ref{ass3}. 
\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{images/assimetria.pdf}
\caption{Separation between \ce{^36Ar} and \ce{^40Ar}  vs. 
the mass flow rate, V, inside the column. Results of the HYSYS simulations, $S^{TF}_{36-40}$ (red dots) and $S^{FB}_{36-40}$ (blue dots));  experimental measurements for run A,B, and C (green and violet triangles).  }
\label{ass3}
\end{figure}
For this  study, we performed the HYSYS simulation with only one set of  input parameter, corresponding to  $p=1.544$ bar   and HETP$=13$ cm. 
%By performing several simulations, the isotopic configuration from top and bottom of the column has been calculated; the separations were then derived from these and added to Fig. \ref{ass3}, together with the experimental results. 
We note that, not only the dependence on the sizing parameter but also the separation asymmetry is reasonably well reproduced by the simulation.  

%It is not clear how to explain the  fluctuations in the measured separations in Run C of Fig. \ref{ass2} since they have different sign and shape in the top and in the bottom.
%From this figure we notice that the experimental results and the simulations show a satisfying congruence considering that they were carried out at different pressures. However, it is clear how the trend as a function of the flow (or sizing parameter) is compatible between theoretical simulations and experimental measurements. The asymmetry decreases as a function of the flow of the column. This is consistent with what was said previously as the increase in the flow of the column moves the various components of the gas and breaks the stagnation of \ce{^40Ar}.

==> sections/capacity.tex <==
\subsection{Useful capacity}
\label{sec:Maximum useful capacity}
\label{tabCp}
The useful capacity of the packing, $\mathrm{C_p}$, is defined as the mass ratio of liquid and vapor.
The maximum useful capacity (also referred to as maximum efficient capacity or maximum operational capacity) is the maximum value  that provides normal efficiency of the packing before reaching  flooding conditions, which leads to  column inefficiency.  
The capacity of the packing depends on the specific geometric area, the specific vapor and liquid loads, and the physical properties, mainly the vapor and liquid densities, the surface tension, and to a lesser extent, on the viscosity of the liquid.
%This operational capacity is usually set by the designers between $0.75$ and $0.85$ of the maximum capacity.
Table \ref{tabCp} shows the  useful capacity  calculated  for the three runs, compared with Sulcol and HYSYS simulation.
During these runs, we are in the minimum conditions, i.e. $\mathrm{C_p}$ is about $25-30\%$,  and therefore very far from the  flooding limit. 
%Also, for this parameter, the results with Sulcol, HYSYS, and our calculation were compared.

\begin{table}
\setlength{\tabcolsep}{21pt}
\centering
\caption{Useful capacity, $\mathrm{C_p}$, calculations for run A, B, and C.}
\begin{tabular}{@{} l l l l @{}}
\hline\noalign{\smallskip}
\multicolumn{4}{c}{\textbf{$\mathrm{C_p} (\%)$ }} \\
\hline\noalign{\smallskip}
 &Sulcol& HYSYS& our estimate \\
%&$(\%)$ &$(\%)$& $(\%)$\\
A&$28.3$&$29.3$&$28.2$\\ 
B&$29.9$&$30.7$&$32.9$\\  
C&$35.2$&$36.4$&$26.5$\\  
\hline
\label{tabCp}
\end{tabular}
\end{table}

The level of agreement among the calculations is remarkable, except for Run C. This is probably due to the fact that we have loaded the column always with $250$ kg of argon, independent  of the vapor mass flow. This loading is sub-optimal for the conditions of run C, which would require more argon, and this leads to a sub-optimal capacity factor.

==> sections/lesson.tex <==
\section{Lessons for the operation of the Aria plant}
\label{sec:calculation39}
\todo[inline]{qui o stimiamo anche la distillazioen con il numero di stadi misurato come lower limit confrotnato questo ideale oppure togliamo il capitolo. parliamone.}
\begin{figure}[htbp]
\centering
\includegraphics[height=7.62cm, width=11.43cm]{images/aggiustato 4.pdf}
\caption{General structure of Seruci-1 distillation column. On the picture are presented the different possible input stages $Nr$ and is highlighted in red the input stage of \cite{Darkside:2021}. \ce{^39Ar}, \ce{^36Ar} and \ce{^38Ar} are expected to increase the concentration in the top of the column and, since we want to reduce the concentration of \ce{^39Ar}, we will extract from the bottom of the column (in blue). The input mass flow $F$ and the concentrations $x_{F,39}$ and $x_{B,39}$ (feed and bottom concentration of \ce{^39Ar}) are presented in the picture as they will be inputs for our simulation}
\label{Hysys2}
\end{figure}
In this section we want to demonstrate numerically that a multicomponent treatment is not necessary in order to simulate the distillation of \ce{^39Ar} under the conditions of Seruci-1. In \ref{Hysys2} is represented the general structure of the distillation column. $x_{D,i}$, $x_{B,i}$,$x_{F,i}$ are the concentration of $i$ component in, respectively, distillate, bottom and feed. $B$, $D$, $F$ are the total (no distinction between different component) mass flows, typically expressed in kg/h. The total number of stage for Seruci-1 is $N=2870$ (HETP$=10$ cm).  \ce{^39Ar}, \ce{^36Ar} and \ce{^38Ar} are expected to increase the concentration in the top of the column and, since we want to reduce the concentration of \ce{^39Ar}, we will extract from the bottom of the column (in blue).
In the following tables are summarized inputs and outputs of \ref{Hysys2}.
\begin{table}[ht]
\centering
\begin{tabular}{c c}
\hline\noalign{\smallskip}
Input & Value\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$x_{F,39}$& $6*10^{-19}$\\ 
$x_{B,39}$& $6*10^{-20}$\\
$L$& $550$ kg/h\\
$T$ & $89.5$ K\\
HETP & $10$ cm\\
$N$ & $2870$\\
$B/F$ & $50\%$\\
\hline
\end{tabular}
\caption{Input values used by \ref{Hysys2} to simulate Seruci-1 }
\end{table}


\begin{table}[ht]
\centering
\begin{tabular}{c c}
\hline\noalign{\smallskip}
Output & Value\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$B$& $0.2804$ kg/h\\ 
$D$&$0.2804$ kg/h\\
$F$& $0.5608$ kg/h\\
$R$& $1995$\\
$x_{D,39}$ & $1.10*10^{-18}$\\
$Nr$ & $574$\\
$R_{D,39}$ & $0.9124$\\
\hline
\end{tabular}
\caption{Output values used by \ref{Hysys2} to simulate Seruci-1. $R_{39,D}$ is the recovery of 39Ar in the top of the column. $R_{D,39}=\frac{D*x_{D,39}}{F*x_{F,39}}$ }
\end{table}
In \cite{Darkside:2021} has been assumed a two components distillation and justified by the following reasons:
\begin{enumerate}
    \item{The concentration of \ce{^36Ar} and \ce{^38Ar} are respectively $0.33\%$ and $0.06\%$, much lower than \ce{^40Ar} ($99,61 1\%$) and higher than \ce{^39Ar} ($10^{-17}\%$).}
    \item{\ce{^36Ar} and \ce{^38Ar} are both lighter than \ce{^39Ar} and thus they are expected to accumulate in the top of column. Since we are extracting from the bottom, they should not bother the measure and the simulation.}
    \item{$x_{B,i}\:<\:1.8\:x_{F,i}$ and $x_{D,i}\:<\: 2.2\:x_{F,i}$ for every isotope $i$. This explains how there cannot be such an enrichment as to make concentrations of 36-Ar and 38-Ar competitive with 40Ar }
\end{enumerate}
Our goal is therefore to compare HYSYS parameters with those already obtained by McCabe-Thiele. HYSYS needs different inputs and therefore we will have to use both some inputs and some outputs of paper \ref{Hysys2} to simulate the same column, finally we will compare the outputs of HYSYS with the remaining parameters of MCT. Inputs and outputs of HYSYS are in the following tables.\\ \\ 

\begin{table}[ht]
\centering
\begin{tabular}{c c}
\hline\noalign{\smallskip}
Input & Value\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$F$& $0.5608$ kg/h\\
$x_{F,39}$& $6*10^{-19}$\\ 
$x_{F,38}$& $6*10^{-4}$\\
$x_{F,36}$& $3.3*10^{-3}$\\
$x_{B,39}$& $6*10^{-20}$\\
$L$& $550$ kg/h\\
$T$ & $89.5$ K\\
$P_c$ & $1.3$ bar\\
HETP & $10$ cm\\
$N$ & $2870$\\
$Nr$ & $574$\\
\hline
\end{tabular} 
\caption{Input values used by HYSYS to simulate Seruci-1. We are in multicomponent condition as also the concentrations of \ce{^38Ar} and \ce{^36Ar} are specified.}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{c c}
\hline\noalign{\smallskip}
Output & Value\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$B$& $0.2642$ kg/h\\ 
$D$&$0.2941$ kg/h\\
$R$& $1874$\\
$R_{D,39}$& $0.9527$\\
$x_{D,39}$ & $1.09*10^{-18}$\\
$x_{D,38}$ & $0.001195$\\
$x_{D,36}$ & $0.006378$\\
$x_{B,38}$ & $1.38*10^{-6}$\\
$x_{B,36}$ & $2.452^{-9}$\\
\hline
\end{tabular}
\caption{Output values used by HYSYS to simulate Seruci-1. }
\end{table}
In all the tables the concentration of \ce{^40Ar} has never been specified as it is always $1-\sum_{i}^{\mathrm{All isotopes}} x_{i}$.\\ \\ Finally we made a two-component simultation with HYSYS, in order to have also an example of rigorous distillation without multicomponent. 

\begin{table}[ht]
\centering
\begin{tabular}{c c}
\hline\noalign{\smallskip}
Input & Value\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$F$& $0.5608$ kg/h\\
$x_{F,39}$& $6*10^{-19}$\\ 
$x_{B,39}$& $6*10^{-20}$\\
$L$& $550$ kg/h\\
$T$ & $89.5$ K\\
$P_c$ & $1.3$ bar\\
HETP & $10$ cm\\
$N$ & $2870$\\
$Nr$ & $574$\\
\hline
\end{tabular}
\caption{Input values used by HYSYS to simulate Seruci-1 with only two components}
\end{table}
\begin{table}[ht]
\centering
\begin{tabular}{c c}
\hline\noalign{\smallskip}
Output & Value\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$B$& $0.2657$ kg/h\\ 
$D$&$0.2963$ kg/h\\
$R$& $1864$\\
$R_{D,39}$& $0.9525$\\
$x_{D,39}$ & $1.09*10^{-18}$\\
\hline
\end{tabular}
\caption{Output values used by HYSYS to simulate Seruci-1, with only two components. }
\end{table}
Finally, we can compare the results of the three cases.

\begin{table}[ht]
\centering
\begin{tabular}{c c c c}
\hline\noalign{\smallskip}
Output & Paper (MCT) & HYSYS multi- & HYSYS two- \\
\noalign{\smallskip}\hline\noalign{\smallskip}
$D$ (kg/h)&\textcolor{red} {$0.2804$} & $0.2941 $ &$0.2926$\\ 
$D$ (kg/day)&\textcolor{red}{$6.73$}&$7.06$&$7.02$\\
$B$ (kg/h)&\textcolor{red} {$0.2804$} &$0.2642$ & $0.2657$\\ 
$B$ (kg/day)&\textcolor{red}{$6.73$}&$6.34$&$6,38$\\
$x_{D,39}$ &\textcolor{red} {$1.10*10^{-18}$}& $1.09*10^{-18}$& $1.09*10^{-18}$\\
$R_{D,39}$&\textcolor{red} {$0.9124$}&$0.9527$&$0.9524$\\
$R$&\textcolor{red}{$1995$}&$1874$&$1864$\\
\hline
\end{tabular}
\caption{Comparison of the results of the paper \ref{Hysys2} (shortcut, 2 components), with HYSYS (rigorous, 2 components and rigorous, multicomponent)  }
\end{table}
Where we notice how the discrepancy among the three cases is acceptable. In particular the difference between HYSYS multi- and two-components is negligible, thus confirming the good agreement between these two cases under these conditions for Seruci-1.\\ \\ In the following table are explicitly represented the percentage discrepancies.
\begin{table}[ht]
\centering
\begin{tabular}{c c c c}
\hline\noalign{\smallskip}
Output & Paper(MCT)-HYSYS discr. & HYSYS multi-two discr. \\
\noalign{\smallskip}\hline\noalign{\smallskip}
${D}$&$4.6\:\%$&$0.51 \%$\\ 
${B}$&$4.6\: \% $&$0.57 \%$\\ 
${x_{D,39}}$ &$0.91\:\%$&$0 \%$\\ 
${R_{D,39}}$&$4.4\:\%$&$0.03 \%$\\ 
${R}$&$6.3\:\%$&$0.53 \%$\\ 
\hline
\end{tabular}
\caption{Discrepancy between the results of the paper \ref{Hysys2} (shortcut, 2 components) and HYSYS) (rigorous, 2 components and rigorous, multicomponent)  }
\end{table}
\\ \\ In the previous tabular we underline how the discrepancy between HYSYS multi- and two- components is systematically smaller than the other one. On the other hand the difference between HYSYS and the results of paper \ref{Hysys2} is more evident but still acceptable. This suggests us that the differences between multi- and two-component distillation are considerably smaller than those between rigorous and shortcut method. In summary, we can affirm that the approximations made in the paper (shortcut and twocomponent) are generally acceptable and that between these two the most relevant is the fact that a rigorous method has not been used.

